Forecasting day-ahead electricity prices: A review of state-of-the-art algorithms, best practices and an open-access benchmark

While the field of electricity price forecasting has benefited from plenty of contributions in the last two decades, it arguably lacks a rigorous approach to evaluating new predictive algorithms. The latter are often compared using unique, not publicly available datasets and across too short and limited to one market test samples. The proposed new methods are rarely benchmarked against well established and well performing simpler models, the accuracy metrics are sometimes inadequate and testing the significance of differences in predictive performance is seldom conducted. Consequently, it is not clear which methods perform well nor what are the best practices when forecasting electricity prices. In this paper, we tackle these issues by performing a literature survey of state-of-the-art models, comparing state-of-the-art statistical and deep learning methods across multiple years and markets, and by putting forward a set of best practices. In addition, we make available the considered datasets, forecasts of the state-of-the-art models, and a specifically designed python toolbox, so that new algorithms can be rigorously evaluated in future studies.

==> discussion.tex <==
In order to discuss the results, we divide this section in three parts respectively comprising an analysis of the metrics, a discussion on state-of-the-art models, and a discussion on the effectiveness of ensemble methods.%, and an analysis of surprising difference in performances between DNNs and LEAR models in the EPEX-FR and EPEX-BE datasets.

\subsection{Metrics}
The obtained results validate the general guideline regarding accuracy metrics:  research in EPF should avoid MAPE and only use metrics like sMAPE in conjunction with any version of \rmae{}. Particularly, the results validate the following three claims:

\begin{itemize}
% 	\item \rmae{} is the best and most reliable metric. First, it ranks the models following the same ranking as the statistical tests. \RW{probably because you are using absolute errors in gwtest.m ...}\JL{But sMAPE and MAPE are also based on the absolute errors, yet their rank is different. Do you think this is not a valid point? On the other hand, absolute errors is what we care most often in terms of economic costs derived from market prices, right?}
% 	In addition, it is a scaled metric so it allows comparisons between different datasets.
	\item MAE is as reliable as \rmae{}. However, as the errors are not relative, comparison between datasets is not possible and \rmae{} is preferred.	
	\item sMAPE is more reliable than MAPE and it mostly agrees with MAE/\rmae{}. Yet, it disagrees with \rmae{} and MAE in one of the four datasets and it has the problem of undefined mean and infinite variance. Thus, it is less reliable than \rmae{}.	
	\item MAPE is not a reliable metric as it gives more importance to datapoints close to zero. As such, using MAPE can lead to misleading results and wrong conclusions.
\end{itemize}


\subsection{State-of-the-art models}
Based on the extensive comparison, it can be concluded that the models based on DL are more likely to outperform those based on statistical methods. This is especially true in the context of  DL ensemble models as the ensemble of DNNs obtains results that are statistically significantly better than any other model. 

However, while DNNs generally outperformed the LEAR models, the latter are still the state-of-the-art in terms of low complexity and computational cost. In particular, their performance is very close to that of DNNs, but with the advantage of having computational costs that are up to 100 times lower. As such, they are the best available option when decision making has to be done within seconds. Hence, new models for EPF should either be compared against LEAR or DNN depending on their computational time. for a method to be considered more accurate than state-of-the-art methods, it should either be more accurate than the DNN model, or more accurate than LEAR but with similar or  lower computational requirements.


% However, the claim might not hold under all circumstances as, in the context of individual models, the LEAR is more accurate than the DNN in one out of the four datasets. Thus, while DNNs seem to perform better, it is important to note that the best performing method will always depend on the dataset under study.

% In that spirit, the datasets, the code of models, and the forecasts of the model are made open-access. By doing so, new statistical and ML models can be evaluated and compared in equal conditions and a better understanding of EPF can be obtained.

\subsection{Ensembles}
The obtained results also validate the claim about ensembles. Particularly, ensembles usually improve the forecasting accuracy and a simple arithmetic average is enough to highly improve the forecasting accuracy. This claim is validated by analyzing the results of the statistical tests: both the ensemble of DNNs and the ensemble of LEAR models are statistically significantly better than all their individual counterparts.

% \subsection{Statistical testing}
% As indicated in the guidelines, performing statistical testing is paramount to obtain a good understand of the performance of the model. In particular, by only using accuracy metrics, it is very hard to separate the performance of the models. 

% For instance, using only accuracy metrics, the comparison between DNNs and LEAR models is not very clear. While the performance of the DNN models appear to be better, the LEAR is better in one dataset. In addition, while a model might appear to be better, the differences in accuracy are hard to quantify and can be insignificant. Using statistical testing we can observe a significant difference in performance between DNNs and LEAR models, and using that difference, we can establish what method works best. The same applies when comparing the two ensembles, or when analyzing the individual DNNs against the ensemble of LEAR models.

% \subsection{EPEX-BE vs EPEX-FR}

% The data employed for the EPEX-BE and EPEX-FR market are very alike. First, when analyzing the price time series depicted in Figure \ref{fig:datasetsbefr}, it seems that the price series of the EPEX-BE and the EPEX-FR are very similar. Moreover, the models of both markets share the same exogenous inputs, i.e.\ day-ahead forecasts of the load and generation in France, and comprise the same time period. 

% Yet, despite these similarities, there is a large difference in terms of which models perform best for each market: while for EPEX-BE the best models are DNNs, for the EPEX-FR LEAR performs best. 

% While a complete analysis of this effect is beyond the scope of the paper, we can try to provide some of the reasons behind it. A possible explanation behind this effect is the fact that the French day-ahead forecasts (the exogenous inputs of both datasets) do not affect equal to both prices. In particular, in the case of Belgium, as the exogenous inputs belong to another country, it could be that the relation with Belgian prices is more nonlinear, e.g.\ some days the French forecasts might not be relevant at all. If that is the case, more complex models like DNNs might perform better in the case of EPEX-BE, but might be overfilling in the case of EPEX-FR.\footnote{Note that this would not be solved by adding Belgian forecasts for the EPEX-BE. As shown in \cite{Lago2018}, the most important inputs for the EPEX-BE are the French generation and load.}

==> figs/neuralnetexample.tex <==
\def\Nin{2}
\def\Nhid{2}
\def\Nhidd{2}
\def\Nout{2}
\setlength{\separ}{2cm}
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50]

\tikzstyle{every pin edge}=[<-,shorten <=1pt]
\tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
\tikzstyle{input neuron}=[neuron, fill=green!40];
\tikzstyle{output neuron}=[neuron, fill=red!50];
\tikzstyle{hidden neuron}=[neuron, fill=blue!50];
\tikzstyle{hidden neuron 2}=[neuron, fill=orange!50];
\tikzstyle{annot} = [text width=4em, text centered]

% Draw the input layer nodes
\foreach \name / \y in {1,...,\Nin}
% This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
\node[input neuron] (I-\name) at (0,-\y) {$x_{\y}$};
\node at (0,-\Nin-1) {$\vdots$};
\node[input neuron] (I-\Nin+1) at (0,-\Nin-2) {$x_{\nin}$};

% Draw the hidden layer nodes
\foreach \name / \y in {1,...,\Nhid}
\path[yshift=0cm]
node[hidden neuron] (H-\name) at (\separ,-\y cm) {$\hid_{1\y}$};
\node at (\separ,-\Nhid-1) {$\vdots$};
\node[hidden neuron] (H-\Nhid+1) at (\separ,-\Nhid-2) {$\hid_{1\nhidn_1}$};


% Draw the hidden layer nodes
\foreach \name / \y in {1,...,\Nhidd}
\path[yshift=0cm]
node[hidden neuron 2] (H2-\name) at (2\separ,-\y cm) {$\hid_{2\y}$};
\node at (2\separ,-\Nhidd-1) {$\vdots$};
\node[hidden neuron 2] (H2-\Nhidd+1) at (2\separ,-\Nhidd-2) {$\hid_{2 \nhidn_2}$};

\foreach \name / \y in {1,...,\Nout}
\path[yshift=0cm]
node[output neuron] (O-\name) at (3\separ,-\y cm) {$y_{\y}$};
\node at (3\separ,-\Nout-1) {$\vdots$};
\node[output neuron] (O-\Nout+1) at (3\separ,-\Nout-2) {$y_{{\nout}}$};

% Draw the output layer node

% Connect every node in the input layer with every node in the
% hidden layer.

%Input to hidden
\foreach \source in {1,...,\Nin}
\foreach \dest in {1,...,\Nhid}
\path (I-\source) edge (H-\dest);

\foreach \dest in {1,...,\Nhid}
\path (I-\Nin+1) edge (H-\dest);
\foreach \source in {1,...,\Nin}
\path (I-\source) edge (H-\Nhid+1);
\path (I-\Nin+1) edge (H-\Nhid+1);


%Hidden to hidden
\foreach \source in {1,...,\Nhid}
\foreach \dest in {1,...,\Nhidd}
\path (H-\source) edge (H2-\dest);

\foreach \dest in {1,...,\Nhidd}
\path (H-\Nhid+1) edge (H2-\dest);
\foreach \source in {1,...,\Nhid}
\path (H-\source) edge (H2-\Nhidd+1);
\path (H-\Nhid+1) edge (H2-\Nhidd+1);

%Hidden to output
\foreach \source in {1,...,\Nhidd}
\foreach \dest in {1,...,\Nout}
\path (H2-\source) edge (O-\dest);

\foreach \dest in {1,...,\Nout}
\path (H2-\Nhidd+1) edge (O-\dest);
\foreach \source in {1,...,\Nhid}
\path (H2-\source) edge (O-\Nout+1);
\path (H2-\Nhidd+1) edge (O-\Nout+1);

% Annotate the layers
\node[annot,above of=H-1, node distance=1cm] (hl) {Hidden layer};
\node[annot,above of=H2-1, node distance=1cm] (hl) {Hidden layer};
\node[annot,above of=I-1, node distance=1cm] {Input layer};
\node[annot,above of=O-1, node distance=1cm] {Output layer};

\node at (3\separ,-\Nout-1) {$\vdots$};
\end{tikzpicture}

==> tables/table_allsingle_fARXEnsemble.tex <==

	\begin{tabular}{ll|ccccccccc}
		&                         & \bfseries{DNN$_{1}$} & \bfseries{DNN$_{2}$} & \bfseries{DNN$_{3}$} & \bfseries{DNN$_{4}$} & \bfseries{fARX$_{364}$} & \bfseries{fARX$_{728}$} & \bfseries{fARX$_{1092}$} & \bfseries{fARX$_{1456}$} & \bfseries{fARX Ens.} \\
		\hline
		\multirow{4}{*}{\bfseries{NP}}  & \bfseries{MASE$_{\mathbf{168}}$}       & \bfseries{0.539} & 0.545          & 0.562          & 0.563          & 0.608              & 0.617              & 0.614               & 0.613               & 0.595                   \\
		& \bfseries{MAE}            & \bfseries{1.721} & 1.74           & 1.796          & 1.798          & 1.942              & 1.97               & 1.962               & 1.96                & 1.902                 \\
		& \bfseries{MAPE\,[\%]}  & \bfseries{5.48}  & 5.58           & 5.64           & 5.79           & 5.98               & 6.16               & 6.03                & 6.04                & 5.89                   \\
		& \bfseries{sMAPE\,[\%]} & \bfseries{4.97}  & 5.04           & 5.22           & 5.19           & 5.54               & 5.61               & 5.57                & 5.57                & 5.42                    \\
		\hline
		\multirow{4}{*}{\bfseries{PJM}} & \bfseries{MASE$_{\mathbf{168}}$}       & 0.375          & \bfseries{0.358} & 0.365          & 0.389          & 0.381              & 0.368              & 0.367               & 0.367               & 0.364                   \\
		& \bfseries{MAE}            & 3.101          & \bfseries{2.956} & 3.015          & 3.216          & 3.15               & 3.043              & 3.036               & 3.037               & 3.011                   \\
		& \bfseries{MAPE\,[\%]}  & 32.85          & 30.54          & 29.31          & 32.24          & 31.14              & \bfseries{29.76}     & 29.37               & 29.05               & 29.58                   \\
		& \bfseries{sMAPE\,[\%]} & 12.17          & \bfseries{11.65}          & 11.96          & 12.51          & 12.36              & 12.05              & 12.14               & 12.24               & 11.98               \\
		\hline
		\multirow{4}{*}{\bfseries{FR}}  & \bfseries{MASE$_{\mathbf{168}}$}       & 0.479          & 0.466          & 0.468          & 0.472          & 0.461              & 0.447              & 0.457               & 0.466               & \bfseries{0.444}              \\
		& \bfseries{MAE}            & 4.313          & 4.194          & 4.211          & 4.251          & 4.154              & 4.028              & 4.114               & 4.199               & \bfseries{3.998 }                 \\
		& \bfseries{MAPE\,[\%]}  & 15.75          & 14.2           & 15.74          & 16.63          & \bfseries{14.16}     & 14.51              & 14.92               & 15.3                & 14.22                 \\
		& \bfseries{sMAPE\,[\%]} & 11.98          & \bfseries{11.69} & 11.84          & 12.05          & 12.49              & 12.17              & 12.59               & 13.19               & 12.15               \\
		\hline
		\multirow{4}{*}{\bfseries{BE}}  & \bfseries{MASE$_{\mathbf{168}}$}       & 0.726          & 0.721          & 0.726          & \bfseries{0.717} & 0.754              & 0.738              & 0.744               & 0.752               & 0.73                \\
		& \bfseries{MAE}            & 6.199          & 6.156          & 6.195          & \bfseries{6.122} & 6.431              & 6.295              & 6.349               & 6.413               & 6.232            \\
		& \bfseries{MAPE\,[\%]}  & 27.66          & 30.25          & 28.31          & 25.9           & 24.76              & \bfseries{23.55}     & 23.83               & 19.7                & 22.13     \\
		& \bfseries{sMAPE\,[\%]} & 14.43          & 14.44          & 14.38          & \bfseries{14.16} & 15.63              & 15.25              & 15.53               & 15.94               & 15.11           
	\end{tabular}

==> tables/table_ensemble_allmetrics.tex <==
	\begin{tabular}{ll|cccc}
		&                         & \textbf{DNN Ensemble} & \textbf{Lasso Ensemble} & \textbf{Best DNN} & \textbf{Best Lasso} \\
		\hline
		\multirow{6}{*}{\textbf{NP}}  & \textbf{MASE}           & \textbf{0.736}        & 0.856                   & 0.775             & 0.874               \\
		& \textbf{MASE 24}        & \textbf{0.709}        & 0.826                   & 0.747             & 0.843               \\
		& \textbf{MASE 168}       & \textbf{0.512}        & 0.595                   & 0.539             & 0.608               \\
		& \textbf{MAE}            & \textbf{1.634}        & 1.902                   & 1.721             & 1.942               \\
		& \textbf{MAPE {[}\%{]}}  & \textbf{5.27}         & 5.89                    & 5.48              & 5.98                \\
		& \textbf{SMAPE {[}\%{]}} & \textbf{4.76}         & 5.42                    & 4.97              & 5.54                \\
		\hline
		\multirow{6}{*}{\textbf{PJM}} & \textbf{MASE}           & \textbf{0.482}                 & {0.5}            & 0.491             & 0.504               \\
		& \textbf{MASE 24}        & \textbf{0.475}                 & {0.493}          & 0.484             & 0.497               \\
		& \textbf{MASE 168}       & \textbf{0.351 }                & {0.364}          & 0.358             & 0.367               \\
		& \textbf{MAE}            & \textbf{2.900}                   & {3.011}          & 2.956             & 3.036               \\
		& \textbf{MAPE {[}\%{]}}  & 30.61                 & 29.58                   & 30.54             & \textbf{29.37}               \\
		& \textbf{SMAPE {[}\%{]}} & \textbf{11.47 }                & 11.98                   & 12.17             & 12.14               \\
		\hline
		\multirow{6}{*}{\textbf{FR}}  & \textbf{MASE}           & \textbf{0.532}                 & 0.539                   & 0.566             & 0.543               \\
		& \textbf{MASE 24}        & \textbf{0.443 }                & 0.449                   & 0.471             & 0.453               \\
		& \textbf{MASE 168}       & \textbf{0.438  }               & 0.444                   & 0.466             & 0.447               \\
		& \textbf{MAE}            & \textbf{3.945 }                & 3.998                   & 4.194             & 4.028               \\
		& \textbf{MAPE {[}\%{]}}  & 14.62                 & 14.22                   & \textbf{14.20}              & 14.51               \\
		& \textbf{SMAPE {[}\%{]}} & \textbf{10.95}                 & {12.15}          & 11.69             & 12.17               \\
		\hline
		\multirow{6}{*}{\textbf{BE}}  & \textbf{MASE}           & \textbf{0.774}                 & 0.819                   & 0.809             & 0.827               \\
		& \textbf{MASE 24}        & \textbf{0.664}                 & 0.703                   & 0.694             & {0.71}       \\
		& \textbf{MASE 168}       & \textbf{0.69}                  & 0.73                    & 0.721             & {0.738}      \\
		& \textbf{MAE}            & \textbf{5.89 }                 & 6.232                   & 6.156             & {6.295}      \\
		& \textbf{MAPE {[}\%{]}}  & {27.19}                 & \textbf{22.13}                   & 30.25             & 23.55               \\
		& \textbf{SMAPE {[}\%{]}} & \textbf{13.53}                 & 15.11                   & 14.44             & {15.25}     
	\end{tabular}

==> tables/table_onlyMASE_allsingle.tex <==
	\begin{tabular}{ll|cccccccc}
	&                         & \bfseries{DNN$_{1}$} & \bfseries{DNN$_{2}$} & \bfseries{DNN$_{3}$} & \bfseries{DNN$_{4}$} & \bfseries{fARX$_{364}$} & \bfseries{fARX$_{728}$} & \bfseries{fARX$_{1092}$} & \bfseries{fARX$_{1456}$} \\
	\hline
	\multirow{3}{*}{\bfseries{NP}}  & \bfseries{MASE$_\mathrm{EPF}$}           & \bfseries{0.775} & 0.783          & 0.809          & 0.809          & 0.874              & 0.887              & 0.884               & 0.882                 \\
	& \bfseries{MASE$_{\mathbf{24}}$}        & \bfseries{0.747} & 0.755          & 0.78           & 0.78           & 0.843              & 0.855              & 0.852               & 0.851                  \\
	& \bfseries{MASE$_{\mathbf{168}}$}       & \bfseries{0.539} & 0.545          & 0.562          & 0.563          & 0.608              & 0.617              & 0.614               & 0.613                 \\
	\hline
	\multirow{3}{*}{\bfseries{PJM}} & \bfseries{MASE$_\mathrm{EPF}$}           & 0.515          & \bfseries{0.491} & 0.501          & 0.534          & 0.523              & 0.506              & 0.504               & 0.505                 \\
	& \bfseries{MASE$_{\mathbf{24}}$}        & 0.507          & \bfseries{0.484} & 0.493          & 0.526          & 0.515              & 0.498              & 0.497               & 0.497              \\
	& \bfseries{MASE$_{\mathbf{168}}$}       & 0.375          & \bfseries{0.358} & 0.365          & 0.389          & 0.381              & 0.368              & 0.367               & 0.367                 \\
	\hline
	\multirow{3}{*}{\bfseries{FR}}  & \bfseries{MASE$_\mathrm{EPF}$}           & 0.582          & 0.566          & 0.568          & 0.573          & 0.56               & \textbf{0.543}              & 0.555               & 0.566                  \\
	& \bfseries{MASE$_{\mathbf{24}}$}        & 0.485          & 0.471          & 0.473          & 0.478          & 0.467              & \textbf{0.453}              & 0.462               & 0.472             \\
	& \bfseries{MASE$_{\mathbf{168}}$}       & 0.479          & 0.466          & 0.468          & 0.472          & 0.461              & \textbf{0.447 }             & 0.457               & 0.466                  \\
	\hline
	\multirow{3}{*}{\bfseries{BE}}  & \bfseries{MASE$_\mathrm{EPF}$}           & 0.815          & 0.809          & 0.814          & \bfseries{0.805}          & 0.845              & 0.827              & 0.834               & 0.843                    \\
	& \bfseries{MASE$_{\mathbf{24}}$}        & 0.699          & 0.694          & 0.699          & \bfseries{0.69}  & 0.725              & 0.71               & 0.716               & 0.723               \\
	& \bfseries{MASE$_{\mathbf{168}}$}       & 0.726          & 0.721          & 0.726          & \bfseries{0.717} & 0.754              & 0.738              & 0.744               & 0.752             \\        
\end{tabular}

==> tables/table_onlyMASE_allsingle_fARXEnsemble.tex <==
	\begin{tabular}{ll|ccccccccc}
		&                         & \bfseries{DNN$_{1}$} & \bfseries{DNN$_{2}$} & \bfseries{DNN$_{3}$} & \bfseries{DNN$_{4}$} & \bfseries{fARX$_{364}$} & \bfseries{fARX$_{728}$} & \bfseries{fARX$_{1092}$} & \bfseries{fARX$_{1456}$} & \bfseries{fARX Ens.} \\
		\hline
		\multirow{3}{*}{\bfseries{NP}}  & \bfseries{MASE$_\mathrm{EPF}$}           & \bfseries{0.775} & 0.783          & 0.809          & 0.809          & 0.874              & 0.887              & 0.884               & 0.882               & 0.856                   \\
		& \bfseries{MASE$_{\mathbf{24}}$}        & \bfseries{0.747} & 0.755          & 0.78           & 0.78           & 0.843              & 0.855              & 0.852               & 0.851               & 0.826                   \\
		& \bfseries{MASE$_{\mathbf{168}}$}       & \bfseries{0.539} & 0.545          & 0.562          & 0.563          & 0.608              & 0.617              & 0.614               & 0.613               & 0.595                   \\
		\hline
		\multirow{3}{*}{\bfseries{PJM}} & \bfseries{MASE$_\mathrm{EPF}$}           & 0.515          & \bfseries{0.491} & 0.501          & 0.534          & 0.523              & 0.506              & 0.504               & 0.505               & 0.5                \\
		& \bfseries{MASE$_{\mathbf{24}}$}        & 0.507          & \bfseries{0.484} & 0.493          & 0.526          & 0.515              & 0.498              & 0.497               & 0.497               & 0.493                \\
		& \bfseries{MASE$_{\mathbf{168}}$}       & 0.375          & \bfseries{0.358} & 0.365          & 0.389          & 0.381              & 0.368              & 0.367               & 0.367               & 0.364                   \\
		\hline
		\multirow{3}{*}{\bfseries{FR}}  & \bfseries{MASE$_\mathrm{EPF}$}           & 0.582          & 0.566          & 0.568          & 0.573          & 0.56               & 0.543              & 0.555               & 0.566               & \bfseries{0.539}                   \\
		& \bfseries{MASE$_{\mathbf{24}}$}        & 0.485          & 0.471          & 0.473          & 0.478          & 0.467              & 0.453              & 0.462               & 0.472               & \bfseries{0.449}                 \\
		& \bfseries{MASE$_{\mathbf{168}}$}       & 0.479          & 0.466          & 0.468          & 0.472          & 0.461              & 0.447              & 0.457               & 0.466               & \bfseries{0.444}              \\
		\hline
		\multirow{3}{*}{\bfseries{BE}}  & \bfseries{MASE$_\mathrm{EPF}$}           & 0.815          & 0.809          & 0.814          & \bfseries{0.805}          & 0.845              & 0.827              & 0.834               & 0.843               & 0.819                \\
		& \bfseries{MASE$_{\mathbf{24}}$}        & 0.699          & 0.694          & 0.699          & \bfseries{0.69}  & 0.725              & 0.71               & 0.716               & 0.723               & 0.703              \\
		& \bfseries{MASE$_{\mathbf{168}}$}       & 0.726          & 0.721          & 0.726          & \bfseries{0.717} & 0.754              & 0.738              & 0.744               & 0.752               & 0.73                \\        
	\end{tabular}

==> tables/table_onlyMASE_allsingle_rank.tex <==
	\begin{tabular}{ll|cccccccc}
	&                         & \bfseries{DNN$_{1}$} & \bfseries{DNN$_{2}$} & \bfseries{DNN$_{3}$} & \bfseries{DNN$_{4}$} & \bfseries{fARX$_{364}$} & \bfseries{fARX$_{728}$} & \bfseries{fARX$_{1092}$} & \bfseries{fARX$_{1456}$} \\
	\hline
	\multirow{3}{*}{\bfseries{NP}}  & \bfseries{MASE$_\mathrm{EPF}$} & 1 & 2& 3& 4 & 5 & 8 & 7 & 6 \\
	& \bfseries{MASE$_{\mathbf{24}}$}        & 1 & 2& 3& 4 & 5 & 8 & 7 & 6              \\
	& \bfseries{MASE$_{\mathbf{168}}$}       & 1 & 2& 3& 4 & 5 & 8 & 7 & 6           \\
	\hline
	\multirow{3}{*}{\bfseries{PJM}} & \bfseries{MASE$_\mathrm{EPF}$} & 6& 1 & 2& 8 & 7& 5&3&4\\
	& \bfseries{MASE$_{\mathbf{24}}$}        & 6& 1 & 2& 8 & 7& 5&3&4   \\
	& \bfseries{MASE$_{\mathbf{168}}$}       & 6& 1 & 2& 8 & 7& 5&3&4  \\
	\hline
	\multirow{3}{*}{\bfseries{FR}}  & \bfseries{MASE$_\mathrm{EPF}$}           & 8    & 4 & 6   & 7 & 3 & 1 & 2  & 5                  \\
	& \bfseries{MASE$_{\mathbf{24}}$}       & 8    & 4 & 6   & 7 & 3 & 1 & 2  & 5                  \\
	& \bfseries{MASE$_{\mathbf{168}}$}      & 8    & 4 & 6   & 7 & 3 & 1 & 2  & 5                         \\
	\hline
	\multirow{3}{*}{\bfseries{BE}}  & \bfseries{MASE$_\mathrm{EPF}$}           & 0.815          & 0.809          & 0.814          & \bfseries{0.805}          & 0.845              & 0.827              & 0.834               & 0.843                    \\
	& \bfseries{MASE$_{\mathbf{24}}$}        & 0.699          & 0.694          & 0.699          & \bfseries{0.69}  & 0.725              & 0.71               & 0.716               & 0.723               \\
	& \bfseries{MASE$_{\mathbf{168}}$}       & 0.726          & 0.721          & 0.726          & \bfseries{0.717} & 0.754              & 0.738              & 0.744               & 0.752             \\        
\end{tabular}

==> tables/table_onlyMASE_allsingle_sorted.tex <==
	\begin{tabular}{l|cccccccc}
		\hline             		
		&\multicolumn{8}{c}{\bfseries{NP}}\\
		\hline             
		 & \bfseries{DNN$_{1}$} & \bfseries{DNN$_{2}$} & \bfseries{DNN$_{3}$} & \bfseries{DNN$_{4}$} & \bfseries{fARX$_{364}$} & \bfseries{fARX$_{1456}$} & \bfseries{fARX$_{1092}$} & \bfseries{fARX$_{728}$} \\
	\hline
	\bfseries{MASE$_\mathrm{EPF}$}           & {0.775} & 0.783          & 0.809          & 0.809          & 0.874              & 0.882             & 0.884               & 0.887           \\
	 \bfseries{MASE$_{\mathbf{24}}$}        & {0.747} & 0.755          & 0.78           & 0.78           & 0.843              & 0.851              & 0.852               & 0.855                 \\
	 \bfseries{MASE$_{\mathbf{168}}$}       & {0.539} & 0.545          & 0.562          & 0.563          & 0.608              &        0.613     & 0.614               &     0.617               \\
	\hline
			\hline             
		&\multicolumn{8}{c}{\bfseries{PJM}}\\
	\hline
	         & \bfseries{DNN$_{2}$} & \bfseries{DNN$_{3}$} & \bfseries{fARX$_{1092}$} & \bfseries{fARX$_{1456}$} & \bfseries{fARX$_{728}$} & \bfseries{DNN$_{1}$} & \bfseries{fARX$_{364}$} & \bfseries{DNN$_{4}$} \\
		\hline
	 \bfseries{MASE$_\mathrm{EPF}$}        &   0.491 & 0.501 & 0.504      & 0.505      & 0.506     & 0.515 & 0.523     & 0.534\\
	 \bfseries{MASE$_{\mathbf{24}}$}        &0.484 & 0.493 & 0.497      & 0.497      & 0.498     & 0.507 & 0.515     & 0.526 \\
	 \bfseries{MASE$_{\mathbf{168}}$}       & 0.358 & 0.365 & 0.367      & 0.367      & 0.368     & 0.375 & 0.381     & 0.389 \\ 
	\hline
\hline             
&\multicolumn{8}{c}{\bfseries{BE}}\\
\hline
& \bfseries{DNN$_{4}$} & \bfseries{DNN$_{2}$} & \bfseries{DNN$_{3}$} & \bfseries{DNN$_{1}$} & \bfseries{fARX$_{728}$} & \bfseries{fARX$_{1092}$} & \bfseries{fARX$_{1456}$} & \bfseries{fARX$_{364}$} \\
\hline
\bfseries{MASE$_\mathrm{EPF}$}           & 0.805 & 0.809 & 0.814 & 0.815 & 0.827     & 0.834      & 0.843      & 0.845     \\
\bfseries{MASE$_{\mathbf{24}}$}        & 0.690 & 0.694 & 0.699 & 0.699 & 0.710     & 0.716      & 0.723      & 0.725     \\
\bfseries{MASE$_{\mathbf{168}}$}       & 0.717 & 0.721 & 0.726 & 0.726 & 0.738     & 0.744      & 0.752      & 0.754              \\   	 
	\hline
		\hline             	
		&\multicolumn{8}{c}{\bfseries{FR}}\\
\hline
    & \bfseries{fARX$_{728}$} & \bfseries{fARX$_{1092}$} & \bfseries{fARX$_{364}$} & \bfseries{DNN$_{2}$} & \bfseries{fARX$_{1456}$} & \bfseries{DNN$_{3}$} & \bfseries{DNN$_{4}$} & \bfseries{DNN$_{1}$} \\
\hline
	 \bfseries{MASE$_\mathrm{EPF}$}           & 0.543     & 0.555      & 0.560     & 0.566 & 0.566      & 0.568 & 0.573 & 0.582  \\
	 \bfseries{MASE$_{\mathbf{24}}$}        & 0.453     & 0.462      & 0.467     & 0.471 & 0.472      & 0.473 & 0.478 & 0.485          \\
	 \bfseries{MASE$_{\mathbf{168}}$}       & 0.447     & 0.457      & 0.461     & 0.466 & 0.466      & 0.468 & 0.472 & 0.479   \\     
\end{tabular}










